Moment Matching Training for Neural Machine Translation: A Preliminary Study

In previous works, neural sequence models have been shown to improve significantly if external prior knowledge can be provided, for instance by allowing the model to access the embeddings of explicit features during both training and inference. In this work, we propose a different point of view on how to incorporate prior knowledge in a principled way, using a moment matching framework. In this approach, the standard local cross-entropy training of the sequential model is combined with a moment matching training mode that encourages the equality of the expectations of certain predefined features between the model distribution and the empirical distribution. In particular, we show how to derive unbiased estimates of some stochastic gradients that are central to the training, and compare our framework with a formally related one: policy gradient training in reinforcement learning, pointing out some important differences in terms of the kinds of prior assumptions in both approaches. Our initial results are promising, showing the effectiveness of our proposed framework.

==> preamble.tex <==
\usepackage{amsmath}

\usepackage{times}
\usepackage{latexsym}

\usepackage{url}

\usepackage{amssymb}

\usepackage{dsfont}

\usepackage{mathtools}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% *************************** Graphics and figures *****************************

\usepackage{adjustbox}
\usepackage{graphicx}

%\usepackage{rotating}
%\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

\usepackage{tikz-qtree}
\usepackage{tikz-dependency}
\usepackage[shortlabels, inline]{enumitem}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}

% *********************************** SI Units *********************************
\usepackage{etoolbox,siunitx} % use this package module for SI units
\robustify\bfseries

% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing as per the
% University guidelines

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% ******************************************************************************
% ************************* User Defined Commands ******************************
% ******************************************************************************

% *********** To change the name of Table of Contents / LOF and LOT ************

%\renewcommand{\contentsname}{My Table of Contents}
%\renewcommand{\listfigurename}{My List of Figures}
%\renewcommand{\listtablename}{My List of Tables}

% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

%\renewcommand{\nomname}{Symbols}


% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% *********************** Configure Draft Mode **********************************

% Uncomment to disable figures in `draft'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


% ******************************** Todo Notes **********************************
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}

% *****************************************************************************
% ******************* Better enumeration my MB*************
\usepackage{enumitem}

% *****************************************************************************
% ******************* Highlighting *************
\usepackage{soul}
\newcommand{\hilight}[1]{\hl{#1}}

% *****************************************************************************
% ******************* Commenting *************
\usepackage{comment}

% *****************************************************************************
% ***************** User-defined Math-related Commands *******************

% for all Chapters 
\newcommand{\ff}{\boldsymbol{f}}
\newcommand{\vg}{\boldsymbol{g}}
\newcommand{\hh}{\boldsymbol{h}}
\newcommand{\hhp}{\boldsymbol{h'}}
\newcommand{\xx}{\boldsymbol{x}}
\newcommand{\xxp}{\boldsymbol{x'}}
\newcommand{\yy}{\boldsymbol{y}}
\newcommand{\Whhp}{\boldsymbol{W}^{(hh')}}
\newcommand{\Whh}{\boldsymbol{W}^{(hh)}}
\newcommand{\Whe}{\boldsymbol{W}^{(he)}}
\newcommand{\Wih}{\boldsymbol{W}^{(ih)}}
\newcommand{\Who}{\boldsymbol{W}^{(ho)}}
\newcommand{\Whpo}{\boldsymbol{W}^{(h'o)}}
\newcommand{\Wauxi}{\boldsymbol{W}^{(ai)}}
\newcommand{\WW}{\boldsymbol{W}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bh}{\boldsymbol{b}^{(h)}}
\newcommand{\bhp}{\boldsymbol{b}^{(h')}}
\newcommand{\bo}{\boldsymbol{b}^{(o)}}
\newcommand{\oo}{\boldsymbol{o}}
\newcommand{\ee}{\boldsymbol{e}}
\newcommand\aux{\ee}
%
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\vh}{\boldsymbol{h}}
\newcommand{\vx}{\boldsymbol{x}}
\newcommand{\vl}{\boldsymbol{l}}
\newcommand{\vI}{\boldsymbol{I}}
\newcommand{\vy}{\boldsymbol{y}}
%\newcommand{\vg}{\boldsymbol{g}}
\newcommand{\vW}{\boldsymbol{W}}
\newcommand{\vb}{\boldsymbol{b}}
\newcommand{\vc}{\boldsymbol{c}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\ve}{\boldsymbol{e}}
\newcommand{\vU}{\boldsymbol{U}}
\newcommand{\vTheta}{\boldsymbol{\Theta}}
\newcommand{\vtheta}{\boldsymbol{\theta}}
\newcommand{\vPhi}{\boldsymbol{\Phi}}
\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\vD}{\boldsymbol{D}}
\newcommand{\vr}{\boldsymbol{r}}
\newcommand{\vX}{\boldsymbol{X}}
\newcommand{\vY}{\boldsymbol{Y}}
%
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand\given[1][]{\:#1\vert\:}
%
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%
\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vo}{\boldsymbol{o}}

\usepackage{amsthm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}

\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    l%
    <{\egroup}%
}
\newcommand*\rot{\multicolumn{1}{R{0}{1em}}}
\newcommand*\rotl{\multicolumn{1}{R{75}{1em}|}}
\newcommand*\rotll{\multicolumn{1}{|R{75}{1em}||}}

\newcommand{\greedydec}{gdec}
\newcommand{\beamdec}{bdec}
\newcommand{\optidec}{EGdec}
\newcommand{\furerank}{full rerank}
\newcommand{\firerank}{filtered rerank}

\newcommand{\zhen}{BTEC}
\newcommand{\tdeen}{TEDTalks}
\newcommand{\wdeen}{WMT}
%\newcommand{\enzh}{en$\rightarrow$zh}
%\newcommand{\tdeen}{TED $\textrm{de}\rightarrow\textrm{en}_{\textrm{'14}}$}
%\newcommand{\wdeen}{WMT $\textrm{de}\rightarrow\textrm{en}_{\textrm{'15}}$}
%\newcommand{\fdeen}{$\textrm{de}\rightarrow\textrm{en}_{\textrm{'14}}$}
%\newcommand{\tende}{$\textrm{en}\rightarrow\textrm{de}_{\textrm{'13}}$}
%\newcommand{\fende}{$\textrm{en}\rightarrow\textrm{de}_{\textrm{'14}}$}

\newcommand{\bleu}{BLEU}
\newcommand{\len}{AvgLen}

\newcommand{\bestss}{\ensuremath{^{\dagger}}}
%\newcommand{\ubold}{\fontseries{b}\selectfont} % renew def. for non-extended bold font
%\robustify\ubold

\newcommand{\boldentry}[1]{%
  \multicolumn{1}{S[table-format=2.2,
                    mode=text,
                    text-rm=\fontseries{b}\selectfont
                   ]}{#1}}
